Two-Buyer Sequential Multiunit Auctions with No Overbidding

We study equilibria in two-buyer sequential second-price (or first-price) auctions for identical goods. Buyers have weakly decreasing incremental values, and we make a behavioural no-overbidding assumption: the buyers do not bid above their incremental values. Structurally, we show equilibria are intrinsically linked to a greedy bidding strategy. We then prove three results. First, any equilibrium consists of three phases: a competitive phase, a competition reduction phase and a monopsony phase. In particular, there is a time after which one buyer exhibits monopsonistic behaviours. Second, the declining price anomaly holds: prices weakly decrease over time at any equilibrium in the no-overbidding game, a fact previously known for equilibria with overbidding. Third, the price of anarchy of the sequential auction is exactly $1 - 1/e$.

==> opposing.tex <==
\begin{tikzpicture}[xscale=10,yscale=2]
\node at (0,0) {};
\node at (1,0) {};
\node (v2) at (0,1.6) {$v_2(k)$};
\node (v4) at (1,1.6) {$v_1(T-k)$};
\node (v5) at (-0.1,0) {};
\node (v6) at (1.1,0) {$k$};
\node (v1) at (0,-0.2) {};
\node (v3) at (1,-0.2) {};

\draw[-,dotted] (1/8,0) edge (1/8,1.6);
\draw[-,dotted] (2/8,0) edge (2/8,1.6);
\draw[-,dotted] (3/8,0) edge (3/8,1.6);
\draw[-,dotted] (4/8,0) edge (4/8,1.6);
\draw[-,dotted] (5/8,0) edge (5/8,1.6);
\draw[-,dotted] (6/8,0) edge (6/8,1.6);
\draw[-,dotted] (7/8,0) edge (7/8,1.6);
\node[below] at (1/8,0) {1};
\node[below] at (2/8,0) {2};
\node[below] at (3/8,0) {3};
\node[below] at (4/8,0) {4};
\node[below] at (5/8,0) {5};
\node[below] at (6/8,0) {6};
\node[below] at (7/8,0) {7};

\node[right] at (1,1.2) {\hspace{-2mm}-\hspace{2mm}\tiny{$1.2$}};
\node[right] at (1,1.1) {\hspace{-2mm}-\hspace{2mm}\tiny{$1.1$}};
\node[right] at (1,1) {\hspace{-2mm}-\hspace{2mm}\tiny{$1$}};

\node at (0,.7) {\hspace{-4mm}\tiny{$.7$}\hspace{2mm}-};
\node at (0,.6) {\hspace{-4mm}\tiny{$.6$}\hspace{2mm}-};
\node at (0,.44) {\hspace{-5.5mm}\tiny{$.44$}\hspace{2mm}-};
\node at (0,.25) {\hspace{-5.5mm}\tiny{$.25$}\hspace{2mm}-};

\draw[-{Latex[length=1.5mm, width=1.5mm]}]  (v1) edge (v2);
\draw[-{Latex[length=1.5mm, width=1.5mm]}]  (v3) edge (v4);
\draw[{Latex[length=1.5mm, width=1.5mm]}-{Latex[length=1.5mm, width=1.5mm]}]  (v5) edge (v6);

\draw[-] (1,1.2) edge (6/8,1.2) {};
\draw[-] (3/8,1.1) edge (6/8,1.1) {};
\draw[-] (3/8,1) edge (0,1) {};
\draw[-] (0,.7) edge (1/8,.7) {};
\draw[-] (3/8,.6) edge (1/8,.6) {};
\draw[-] (3/8,.44) edge (6/8,.44) {};
\draw[-] (1,.25) edge (6/8,.25) {};

\draw[domain=0:.375,dashed,variable=\x,blue] plot ({\x},{(5.2-8*\x)/(8-8*\x)});
\draw[domain=.375:.7,dashed,variable=\x,blue] plot ({\x},{(2.2-1.1*(8*\x-3))/(8-8*\x)});

\end{tikzpicture}













==> valuations.tex <==
\begin{tikzpicture}
\usetikzlibrary{arrows.meta}
\node (v1) at (0,-2) {};
\node [scale = 3] (v2) at (0,13){$v_1(k|\0)$};
\node (v3) at (-7,0) {};
\node [scale = 3] (v4) at (12,0) {$k$};

\draw[-{Latex[length=5mm, width=5mm]}]  (v1) edge (v2);
\draw[-{Latex[length=5mm, width=5mm]}]  (v3) edge (v4);
\draw[fill=lightgray]  (0,0) rectangle (2,20/3+1);
\draw[fill=lightgray]  (2,0) rectangle (4,5+1);
\draw[fill=lightgray]  (4,0) rectangle (6,1);
\draw[dashed]  (6,0) rectangle (8,1);
\draw[dashed]  (8,0) rectangle (10,1);
\draw[dashed]  (-2,0) rectangle (0,11);
\draw[dashed]  (-4,0) rectangle (-2,11);
\draw[dashed]  (-6,0) rectangle (-4,11);

\node (v5) at (0+20,-2) {};
\node [scale = 3] (v6) at (0+20,13) {$v_1(k|(-1,1))$};
\node (v7) at (-7+20,0) {};
\node [scale = 3] (v8) at (12+20,0) {$k$};

\draw[-{Latex[length=5mm, width=5mm]}]  (v5) edge (v6);
\draw[-{Latex[length=5mm, width=5mm]}]  (v7) edge (v8);
\draw[fill=lightgray]  (20,0) rectangle (22,11);
\draw[fill=lightgray]  (22,0) rectangle (24,20/3+1);
\draw[fill=lightgray]  (24,0) rectangle (26,5+1);
\draw[dashed]  (26,0) rectangle (28,1);
\draw[dashed]  (28,0) rectangle (30,1);
\draw[dashed]  (18,0) rectangle (20,11);
\draw[dashed]  (16,0) rectangle (18,11);
\draw[dashed]  (14,0) rectangle (16,11);

\end{tikzpicture}
